Light yield and radiation hardness studies of scintillator strips with a filler

Detectors based on polystyrene scintillator strips with WLS fiber readout are widely used to register charged particles in many high-energy physics experiments. The fibers are placed into grooves or holes along the strip. The detection efficiency of these devices can be significantly increased by improving the optical contact between the scintillator and the fiber by adding an optical filler into the groove/hole. This work is devoted to the study of the light yield of a 5-m-long scintillator strip with a 1.2-mm-diameter Kuraray Y11(200)~MC WLS fiber inserted into the strip's co-extruded hole filled with synthetic silicon resin SKTN-MED(E). The light yield was studied using cosmic muons and a $^{60}$Co radioactive source. Radiation hardness study of viscous fillers and short strip samples were performed on the IBR-2 pulsed research reactor of fast neutrons at JINR.

==> text/RadhardScintEng.tex <==
Study of properties for polystyrene samples with similar composition as in ones considered above shows that these samples have good long-term stability of its properties under natural conditions (normal temperature and humidity). Losses in light output did not exceed 20\% for 10~year period \cite{scintUPS923a, scintCDFaging} (see table \ref{table: Act2003}, \ref{App}; \cite{Grinev}). However, these scintillators suffer significant losses in light output at temperatures above $65\: ^{\circ}C$  (figure~ \ref{fig: scinttemp}), and the elevated humidity leads to the formation of microcracks, to the cracking and yellowing of the scintillator; and this as a consequence leads to the light output deterioration due to the scattering and absorption of light \cite{Senchishin}. Number of defects (cracks) created on the strip by exposition time with a humidity level of 95\% at various temperature as function of time exposed is shown in figure \ref{fig: scintdef}.

\begin{figure}[!htbp]
	\centering
	\subfloat[]{\includegraphics[height=0.2\textheight, keepaspectratio]
		{figures/scintTempaging.png} \label{fig: scinttemp} }
	\hfill
	\subfloat[]{\includegraphics[height=0.2\textheight, keepaspectratio]
		{figures/scintTempdefects.png} \label{fig: scintdef} }
	\caption{\small Strip light output dependence by time exposed with various temperature (a)  an number of defects (cracks) created on the strip by exposition time with a humidity level of 95\% at various temperature (b) \cite{Senchishin}.}
	\label{fig: scinttempaging}
\end{figure}

Light transition study as a function on dose rate were done in many articles (for instance, at \cite{zorn93, britvich93, radneutron, vara00, radwls91}).

In polystyrene scintillators, fast neutrons could knock protons from atomic nuclei out by the collisions with them and can produce of $\gamma-$particles as well; these particles could have an energy of few MeV. Such protons have very short path on the polystyrene whereas $\gamma-$particles mainly leave relative thin strips without noticeable interaction, and, due to it, the damage caused by neutrons (protons) is more presented than by $\gamma-$particles. This was noted at article \cite{radneutron}: neutrons caused much higher damage to scintillator SCSN38, 5-times more, against $\gamma-$particles in case of approximate equal irradiation dose rate of: 5.2~kGy for neutron case and 7.0~kGy for $\gamma-$particles case.

Polystyrene transparency changes after irradiation by various dozes are presented on figure \ref{fig: scintraddam}: instantly after irradiation (\ref{fig: scintraddam01}) and after recovery on air (\ref{fig: scintraddam02}) \cite{zorn93}

\begin{figure}[!htbp]
	\centering
	\subfloat[]{\includegraphics[height=0.2\textheight, keepaspectratio]
		{figures/scintraddam01.png} \label{fig: scintraddam01} }
	\hfill
	\subfloat[]{\includegraphics[height=0.2\textheight, keepaspectratio]
		{figures/scintraddam02.png} \label{fig: scintraddam02} }
	\caption{\small Polystyrene transparency changes after irradiation by various dozes: instantly after irradiation (а) and after recovery on air (б) \cite{zorn93}}
	\label{fig: scintraddam}
\end{figure}

Deterioration of WLS fiber's properties under the radiation were discussed at follow articles \cite{vara00, radwls91}. The table \ref{table: wlsradam} taken from article \cite{vara00} presents results of test for Kuraray Y11(200) MC WLS fibers, which were irradiated by $^{60}Co$ with dose rate of 1.16~kGy and 6.93~kGy. Light yield losses for these fibers were occur of 13\% and 29\% instantly after irradiation, and of 9\% and 26\% after 10 days for recovery \cite{vara00}, respectively.

\begin{table}[htb]
\small
  \begin{center}
		\begin{tabular}{|c|c|c|c|c|c|c|}
			\hline
			Fiber 	& \multicolumn{3}{c|}{$\frac{R(140)}{R(30)}$ for 1.16 kGy} & \multicolumn{3}{c|}{$\frac{R(140)}{R(30)}$ for 6.93 kGy}  \\
			\cline{2-7}
			type					& 0 days & 1 day & 10 days & 0 days & 1 day & 10 days \\
		\hline
		BCF91A MC		& 0.83 & 0.86 & 0.85 & 0.54 & 0.56 & 0.56 \\
		Y11(200)MSJ & 0.87 & 0.92 & 0.91 & 0.71 & 0.72 & 0.74 \\
		S250-100 		& 0.60 & 0.70 & 0.81 & 0.52 & 0.55 & 0.64 \\
		\hline

		\end{tabular}
  \end{center}
  \caption{Relative light output at $x = 140$ cm, with total doses of 1.16 and 6.93 kGy \cite{vara00} }
	\label{table: wlsradam}
\end{table}

==> text/Radhardglue.tex <==
Generally, the WLS fibers are glued to a plastic scintillator to improve the light yield. Radiation hardness of the adhesives used has also the huge importance to create the detector with long-term stable parameters.

Study of radiation hardness for various optical glues: Meltmount (thermoplastic), Naphrax (solvent based), Dirax (natural resin) and ВС-600 (epoxy resin) - is presented at article \cite{radcms}. Meltmount I011-1582 \cite{Meltmount}, Naphrax \cite{Naphrax} and Dirax \cite{Dirax} are used in microscopes to couple different optical elements. Study of transmission damage was done for thin samples of glues with thick of 1.5 and 3.0 mm. ВС-600 and Dirax were irradiated with $\gamma-$particles emitted by $^{60}Co$ for the dose rate of 27 kGy, а Meltmount - $\gamma-$particles emitted by $^{60}Co$ and dose rate of 4 kGy; and irradiated by neutron and protons beams with fluencies of $2\times10^{13}$ per cm$^2$ \cite{radcms}. Results of these studies are presented on figure \ref{fig: radinvest}.

\begin{figure}[!htbp]
	\begin{minipage}[h]{0.31\linewidth}
		\center{\includegraphics[width=1\linewidth, keepaspectratio]{figures/radbc600.png}} a) ВС-600 \\
	\end{minipage}
	\hfill
	\begin{minipage}[h]{0.31\linewidth}
		\center{\includegraphics[width=1\linewidth, keepaspectratio]{figures/raddirax.png}} \\b) Dirax
	\end{minipage}
	\vfill
	\begin{minipage}[h]{0.31\linewidth}
		\center{\includegraphics[width=1\linewidth, keepaspectratio]{figures/radmeltmount.png}} c) Meltmount I011-1582 \\
	\end{minipage}
	\hfill
	\begin{minipage}[h]{0.31\linewidth}
		\center{\includegraphics[width=1\linewidth, keepaspectratio]{figures/radnaphrax.png}} d) Naphrax\\
	\end{minipage}
	\caption{\small Transmittance for ВС-600, Meltmount I011-1582, Naphrax glues with various thickness $d$ of samples before and after irradiation \cite{radcms}. Dose rates are displayed on the picture.}
	\label{fig: radinvest}
\end{figure}

% \begin{figure}[!htbp]
%   \centering
%   \subfloat[ВС-600]{\includegraphics[ width=0.23\textwidth, keepaspectratio]
% 			{ }
%   \hfill
%  \subfloat[Dirax]{\includegraphics[width=0.23\textwidth, keepaspectratio]
% 			} }
%   \hfill
%  \subfloat[Meltmount I011-1582]{\includegraphics[width=0.23\textwidth, keepaspectratio]
% 			{} }
%   \hfill
% 	\subfloat[Naphrax]{\includegraphics[width=0.23\textwidth, keepaspectratio]
% 			{} }
%   \caption{}
% 	\label{}
% \end{figure}

One can see that BC-600 glue based on epoxy resin has a bad radiation hardness;
the sharp deterioration of the optical properties has a place in working region of scintillator.



